Formal Proofs of Transcendence for e and $\pi$ as an Application of Multivariate and Symmetric Polynomials

We describe the formalisation in Coq of a proof that the numbers e and $\pi$ are transcendental. This proof lies at the interface of two domains of mathematics that are often considered separately: calculus (real and elementary complex analysis) and algebra. For the work on calculus, we rely on the Coquelicot library and for the work on algebra, we rely on the Mathematical Components library. Moreover, some of the elements of our formalized proof originate in the more ancient library for real numbers included in the Coq distribution. The case of $\pi$ relies extensively on properties of multivariate polynomials and this experiment was also an occasion to put to test a newly developed library for these multivariate polynomials.

==> lstcoq.tex <==
\lstdefinelanguage{Coq} {
% Anything betweeen $ becomes LaTeX math mode
mathescape=true,						

% Comments may or not include Latex commands
texcl=false,

% Vernacular commands
morekeywords=[1]{
  Add,
  All,
  Arguments,
  Axiom,
  Bind,
  Canonical,
  Close,
  CoFixpoint,
  CoInductive,
  Coercion,
  Contextual,
  Corollary,
  Defined,
  Definition,
  Delimit,
  End,
  Example,
  Export,
  Fact,
  Fixpoint,
  Goal,
  Graph,
  Hint,
  Hypotheses,
  Hypothesis,
  Implicit,
  Implicits,
  Import,
  Inductive,
  Lemma,
  Let,
  Local,
  Locate,
  Ltac,
  Maximal
  Module,
  Morphism,
  Notation,
  Open,
  Parameter,
  Parameters,
  Prenex,
  Print,
  Printing,
  Projections,
  Proof,
  Proposition,
  Qed,
  Record,
  Relation,
  Remark,
  Require,
  Reserved,
  Resolve,
  Rewrite,
  Save,
  Scope,
  Search,
  Section,
  Set,
  Show,
  Strict,
  Structure,
  Tactic,
  Theorem,
  Unset,
  Variable,
  Variables,
  View,
  inside,
  outside
},

% Gallina
morekeywords=[2]{
  as,
  cofix,
  else,
  end,
  exists,
  exists2,
  fix,
  for,
  forall,
  fun,
  if,
  in,
  is,
  let,
  match,
  nosimpl,
  of,
  return,
  struct,
  then,
  with
},

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics,
morekeywords=[4]{
  after,
  apply,
  assert,
  auto,
  bool_congr,
  case,
  change,
  clear,
  compute,
  congr,
  cut,
  cutrewrite,
  destruct,
  elim,
  field,
  fold,
  generalize,
  have,
  hnf,
  induction,
  injection,
  intro,
  intros,
  inversion,
  left,
  loss,
  move,
  nat_congr,
  nat_norm,
  pattern,
  pose,
  refine,
  rename,
  replace,
  revert,
  rewrite,
  right,
  ring,
  set,
  simpl,
  split,
  suff,
  suffices,
  symmetry,
  transitivity,
  trivial,
  unfold,
  unlock,
  using,
  without,
  wlog,
  autorewrite
},        

% Terminators
morekeywords=[5]{
  assumption,
  by,
  contradiction,
  done,
  exact,
  lia,
  gappa,
  omega,
  reflexivity,
  romega,
  solve,
  tauto,
  discriminate,
  unsat
},

% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",

% Size of tabulations
tabsize=3,							

% Enables ASCII chars 128 to 255
extendedchars=true,  		 		

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,							

% Full flexible columns 
columns=[l]fullflexible,

% Style for (listings') identifiers
identifierstyle={\color{black}},

% Style for declaration keywords
keywordstyle=[1]{\color{violet}},

% Style for gallina keywords
keywordstyle=[2]{\color{green!50!black}},

% Style for sorts keywords
keywordstyle=[3]{\color{blue}},

% Style for tactics keywords
keywordstyle=[4]{\color{blue}},

% Style for terminators keywords
keywordstyle=[5]{\color{red}},

%Style for iterators
keywordstyle=[6]{\color{violet}},

% Style for strings
stringstyle=,

% Style for comments
commentstyle=,

% Style for lines numbering
numberstyle=\tiny,
}

